On a class of poly-context-free groups generated by automata

This paper deals with graph automaton groups associated with trees and some generalizations. We start by showing some algebraic properties of tree automaton groups. Then we characterize the associated semigroup, proving that it is isomorphic to the partially commutative monoid associated with the complement of the line graph of the defining tree. After that, we generalize these groups by introducing the quite broad class of reducible automaton groups, which lies in the class of contracting automaton groups without singular points. We give a general structure theorem that shows that all reducible automaton groups are direct limit of poly-context-free groups which are virtually subgroups of the direct product of free groups; notice that this result partially supports a conjecture by T. Brough. Moreover, we prove that tree automaton groups with at least two generators are not finitely presented and they are amenable groups, which are direct limit of non-amenable groups.

==> environ.sty.tex <==
%% environ.sty
%% Layout definitions for the Book of Involutions

%% This is for reminders
%% comment in the final version
%\newcommand{\REM}[1]{\marginpar{\tt\raggedright#1}%
%\message{^^JReminder on input line \the\inputlineno: #1^^J}}
%\newcommand{\REF}[1]{\REM{Reference missing: #1}}
%\newcommand{\CITE}[2][]{[000]\REM{Citation missing: #1\space#2}}
%%\newenvironment{typett}{\ttfamily\rightskip 0pt plus100em}{\par}

%% \S sign in text with a little extra space.
%% \Sorig is original version, used at several places
\newcommand{\Sorig}{}\let\Sorig\S
\renewcommand{\S}{\Sorig\kern0.1em\ignorespaces}

%%% TABLE OF CONTENTS

%% subsections in tableofcontents
\setcounter{tocdepth}{2}

%% Here seems to be a bug in amsbook.cls
%% Although we don't need \tocparagraph, it will be written to .aux
%% Although we don't need \tocparagraph, it will be read from .aux
%% Since \tocparagraph and \l@paragraph are not defined, we get errors
\def\l@paragraph{\@tocline{4}{0pt}{1pc}{7pc}{}}
\let\tocparagraph\tocsubsubsection

%%  layout of table of contents:
\renewcommand{\tocchapter}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1
      #2. \quad\vadjust{\nobreak\smallskip}}}#3}
\renewcommand{\tocsection}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1
      \rlap{\Sorig\kern0.1em #2.}\hphantom{\Sorig\ 00. }}}#3}
\renewcommand{\tocsubsection}[3]{%
  \indentlabel{\@ifnotempty{#2}{\ignorespaces#1
      \hphantom{\Sorig\ 00. }\rlap{#2.}\hphantom{00.B. }}}#3}

%% a bad trick to have \goodbreak before chapters in toc
%%\def\l@chapter{\@tocline{0}{8pt plus5pt\goodbreak}{0pt}{}{}}
\def\l@chapter{\@tocline{0}{8pt plus5pt minus 8pt\goodbreak}{0pt}{}{}}
\def\l@section{\@tocline{1}{0pt\penalty-250}{1pc}{}{}}

%% dotted lines \BOOKtocdots in toc
\newcommand{\BOOKtocdots}{\leaders\hbox to 1em{\hss.\hss}}
%% edited from amsbook.cls
\def\@tocline#1#2#3#4#5#6#7{\relax
  \ifnum #1>\c@tocdepth % then omit
  \else
    \par \addpenalty\@secpenalty\addvspace{#2}%
    \begingroup \hyphenpenalty\@M
    \@ifempty{#4}{%
      \@tempdima\csname r@tocindent\number#1\endcsname\relax
    }{%
      \@tempdima#4\relax
    }%
    \parindent\z@ \leftskip#3\relax \advance\leftskip\@tempdima\relax
    \rightskip\@pnumwidth plus1em \parfillskip-\@pnumwidth
    #5\leavevmode\hskip-\@tempdima #6\relax
%% change:
    \BOOKtocdots
%%
    \hfil\hbox to\@pnumwidth{\@tocpagenum{#7}}\par
    \nobreak
    \endgroup
  \fi}

%%%  BIBLIOGRAPHY
%% in case \cite with optional arg appears in an optional arg
%% e.g., \begin{thm}[\cite[Theorem 5, p.~26]{Jacexcep}] does not work,
%% but \begin{thm}[\Cite{Theorem 5, p.~26}{Jacexcep}] works
\newcommand{\Cite}[1]{\cite[#1]}

%% no bold numbers in citation
\def\@cite#1#2{{%
 \m@th\upshape\mdseries[{\relax #1}{\if@tempswa, #2\fi}]}}

%% biblabel, bibsep as in amsplain
\def\bibliographystyle#1{%
  \if@filesw\immediate\write\@auxout
  {\string\bibstyle{#1}}\fi
  \def\@biblabel##1{##1.}%
  \def\bibsetup{}%
  }

%% the rest is for the pagenumbers in the bibliography
%%
\newcommand{\@citextra}[1]{\index{P}{#1}}
\newcommand{\old@citex}{} \let\old@citex\@citex
\def\@citex[#1]#2{\old@citex[{#1}]{#2}\@citextra{#2}}

%% \finbibitem will be inserted in .bbl by boi.bst
\newcommand{\finbibitem}[1]{%
  \expandafter\ifx\csname#1@pages\endcsname\relax
  \else
  \ {\itshape\csname#1@pages\endcsname.}%
  \fi}

%% \bibpagesentry will be inserted in P.ind by boi-P.ist
\newcommand{\bibpagesentry}[2]{%
  \expandafter\gdef\csname#1@pages\endcsname{#2}}

\renewcommand{\thebibliography}[1]{%
  %% no bibpages for citations in the bibliography
  \renewcommand{\@citextra}[1]{}%
  \@input{P.ind}%
  \@xp\chapter\@xp*\@xp{\bibname}%
  \normalfont\footnotesize\labelsep .5em\relax
  %% some preliminary text
  \the\bibliopreliminary
  \renewcommand\theenumiv{\arabic{enumiv}}\let\p@enumiv\@empty
  \list{\@biblabel{\theenumiv}}{\settowidth\labelwidth{\@biblabel{#1}}%
    \leftmargin\labelwidth \advance\leftmargin\labelsep
    \usecounter{enumiv}}%
  \sloppy \clubpenalty\@M \widowpenalty\clubpenalty
  \sfcode`\.=\@m
  %% the parskip avoids underfull \vboxes
  \parskip=0pt plus 1pt \relax
}
\newcommand{\bibliopreliminary}{}
\newtoks\bibliopreliminary

%%%  INDEX
%% multiple standard amsbook index, taken from multind.sty by F. W. Long
\renewcommand{\printindex}[2]{\def\indexname{#2}\@input{#1.ind}}%
\def\makeindex#1{\begingroup
  \makeatletter
  \if@filesw \expandafter\newwrite\csname #1@idxfile\endcsname
  \expandafter\immediate\openout \csname #1@idxfile\endcsname #1.idx\relax
  \typeout{Writing index file #1.idx }\fi \endgroup}
\def\index#1{\@bsphack\begingroup
               \def\protect##1{\string##1\space}\@sanitize
               \@wrindex{#1}}
\def\@wrindex#1#2{\let\thepage\relax
   \xdef\@gtempa{\@ifundefined{#1@idxfile}{}{\expandafter
      \write\csname #1@idxfile\endcsname{\string
      \indexentry{#2}{\thepage}}}}\endgroup\@gtempa
   \if@nobreak \ifvmode\nobreak\fi\fi\@esphack}

%% index{A}: Index
%% index{B}: Notations
%% here we do a \raggedright (via indexstyle BoI-B.ist)
%% this inhibits hyphenations (and overfull \hboxes)
%% \rightskip=0pt plus 2pt would be an alternative
%% index{P}: auxiliary index for the pagenumbers in the bibliography

%%%  GENERAL LAYOUT

%% the parskip has in plain-tex or latex some stretch (plus 1pt)
%% but not in amslatex.
%% The stretch seems to be appropriate in parts which consist
%% mainly of text (no displays, etc.).
%% We give the stretch at the beginning of each chapter,
%% but this will be reset after the first section.
%% Moreover Notes have the stretch.

\def\chapter{\parskip=0pt plus 1pt
  \cleardoublepage \thispagestyle{plain}\global\@topnum\z@
  \@afterindenttrue \secdef\@chapter\@schapter}

%% all numbers (for sections, footnotes, etc.)
%% are independent from chapternumbers
\def\cl@chapter{}
%%\@addtoreset{footnote}{chapter} % in case we want to change back

%% no numberings of subsubsections
\setcounter{secnumdepth}{2}

%% chapternumbers are in Roman letters
\renewcommand{\thechapter}{\Roman{chapter}}

%% sections have a \S sign
\def\section{\parskip=0pt\@startsection{section}{1}%
  \z@{.7\linespacing\@plus\linespacing}{.5\linespacing}%
  {\normalfont\bfseries\centering\Sorig}}
\def\sectionrunhead#1#2#3{%
  \@ifnotempty{#2}{\uppercase{\Sorig#1#2}\@ifnotempty{#3}{. }}%
  \def\@tempa{#3}%
  \ifx\@empty\@tempa\else\uppercasenonmath\@tempa\@tempa\fi}

%% subsectionnumbers are from capital alphabet
\renewcommand{\thesubsection}{\thesection.\Alph{subsection}}

%% subsubsections bold with little vertical space
%% edited from amsbook.cls
\def\subsubsection{\@startsection{subsubsection}{3}%
  \normalparindent{.2\linespacing\@plus.2\linespacing}{-.5em}%
  {\normalfont\bfseries}}

%%%  THMS

%%% theorems
\numberwithin{equation}{section}
\theoremstyle{plain} %
\newtheorem*{thmA}{Theorem} % In chapter I
\newtheorem{thm}[equation]{Theorem}
\newtheorem{prop}[equation]{Proposition}
\newtheorem{cor}[equation]{Corollary}
\newtheorem{lem}[equation]{Lemma}
\theoremstyle{definition} %
\newtheorem{example}[equation]{Example}
\newtheorem{examples}[equation]{Examples}
\newtheorem{remark}[equation]{Remark}
\newtheorem{remarks}[equation]{Remarks}
\newtheorem{defn}[equation]{Definition}
\newtheorem{defns}[equation]{Definitions}
\newtheorem*{claim}{Claim}

%%% thmslayout: use of \newtheoremstyle seems not convenient
%%  better edit the definitions from amsthm.sty

%% start with number in brackets
\def\thmhead@plain#1#2#3{%
  \thmnumber{\@ifnotempty{#1}{}(#2) }\thmname{#1}%
  \thmnote{ \textmd{\upshape(#3)}}}

%% thms in bold
\def\th@plain{%
%%  \let\thm@indent\indent
%%  \thm@headfont{\scshape}% heading font small caps
  \let\thm@indent\relax
  \thm@headfont{\bfseries}% heading bold
%%
  \let\thmhead\thmhead@plain \let\swappedhead\swappedhead@plain
  \thm@preskip.5\baselineskip\@plus.2\baselineskip
                                    \@minus.2\baselineskip
  \thm@postskip\thm@preskip
  \itshape
}
%% definitions in bold
\def\th@definition{%
%%  \let\thm@indent\indent
%%  \thm@headfont{\scshape}% heading font small caps
  \let\thm@indent\relax
  \thm@headfont{\bfseries}% heading bold
%%
  \let\thmhead\thmhead@plain \let\swappedhead\swappedhead@plain
  \thm@preskip.5\baselineskip\@plus.2\baselineskip
                                    \@minus.2\baselineskip
  \thm@postskip\thm@preskip
  \upshape
}
%% \thm@headpunct after \thmnote not bold
\def\@begintheorem#1#2[#3]{%
  \item[\normalfont % reset in case body font is abnormal
  \hskip\labelsep
  \the\thm@headfont
  \thm@indent
  \@ifempty{#1}{\let\thmname\@gobble}{\let\thmname\@iden}%
  \@ifempty{#2}{\let\thmnumber\@gobble}{\let\thmnumber\@iden}%
  \@ifempty{#3}{\let\thmnote\@gobble}{\let\thmnote\@iden
    \thm@headpunct{\textmd{\upshape.}}}%
  \thm@swap\swappedhead\thmhead{#1}{#2}{#3}%
  \the\thm@headpunct]%
  \@restorelabelsep
  \thmheadnl % possibly a newline.
  \ignorespaces}

%% For upshape paranthesis and colon ():
\newcommand{\upp}{} \let\upp\textup

%% equation numbers in bold, edited from amsmath.sty
%%\def\tagform@#1{\maketag@@@{\bf(\ignorespaces#1\unskip)}}
%% the \boldmath is only for \tag{$*$} in Chap.1
\def\tagform@#1{\maketag@@@{\bfseries\boldmath(\ignorespaces#1\unskip)}}

%% \ref's
\newcommand{\OLDref}{} \let\OLDref\ref
%% \ref in upshape
\renewcommand{\ref}[1]{\textup{\OLDref{#1}}}
%% \eqref = (\ref) ref's to equations
\def\eqref#1{\textup{(\OLDref{#1})}}
%% \thmref was introduced for ref's to thms but not to equations
%% But there was never a difference between \eqref and \thmref
%% \thmref has not been used everywhere
\newcommand{\thmref}{} \let\thmref\eqref
%% \Eqref for referencing Lemma (30.2.1) with Lemma~\Eqref{label1}{label2}
\newcommand{\Eqref}[2]{\textup{(\OLDref{#1}.\OLDref{#2})}}

%%% proofs
%% edited from amsbook.cls
\renewenvironment{proof}[1][Proof]{\par \normalfont
  \topsep6\p@\@plus6\p@ \trivlist \itemindent0pt%\normalparindent
  \item[\hskip\labelsep\itshape%\scshape
    #1\/\upshape\@addpunct{:}]\ignorespaces
}{%
  \qed\endtrivlist
  \par  % the \par is new
}
%% proofitem
\newcommand{\pitem}{} \def\pitem#1:{#1\Enspace\ignorespaces}
%% if \end{proof} does not end the proof
\newcommand{\noqed}{\let\qed\relax}

%%%  LISTINGS

\renewcommand{\labelenumi}{\textup{(\theenumi)}}
\renewcommand{\theenumi}{\arabic{enumi}}
\renewcommand{\labelenumii}{\textup{(\theenumii)}}
\renewcommand{\theenumii}{\alph{enumii}}
\renewcommand{\p@enumii}{} % Use \Eqref instead

%% Space after the numbers
%% width {(0)\hskip\standardlabelwidth} = \parindent
\newdimen{\standardlabelwidth}
\settowidth{\standardlabelwidth}{\textup{(0)}}
\standardlabelwidth-\standardlabelwidth
  \advance\standardlabelwidth by \normalparindent
\newcommand{\standardlabel}[1]{#1\kern\standardlabelwidth}
%%\standardlabelwidth = 5.22218pt
%% Use it also in \pitem
\newcommand{\Enspace}{\kern\standardlabelwidth}

%% listings in text
%% like a standard enumerate
\newenvironment{enumerateT}{%
\renewcommand{\theenumi}{\alph{enumi}}%
\setlength{\labelsep}{5pt}%
\settowidth\leftmargini{\textup{(a)}\hskip\labelsep}%
  \advance\leftmargini by \normalparindent
\begin{enumerate}
\labelwidth=\leftmargini \advance\labelwidth-\labelsep
}{\end{enumerate}}

%% listings in theorems
%% Just like usual text with \par\noindent for each item
%% The labels should be leftflush, like the equation numbers
\newenvironment{enumerateA}{%
\setlength{\labelsep}{0pt}%
\setlength{\leftmargini}{0pt}%
\begin{enumerate}%
\renewcommand{\makelabel}{\standardlabel}%
\setlength{\labelwidth}{0pt}%
\setlength{\itemindent}{0pt}%
}{\end{enumerate}}

%% sublistings in theorems
%% the same as \enumerateT, but for use
%% inside \enumerateA or equivalent ones
\newenvironment{enumerateAa}
{\setlength{\labelsep}{5pt}%
\settowidth\leftmarginii{\textup{(a)}\hskip\labelsep}%
  \advance\leftmarginii by \normalparindent
\begin{enumerate}
\labelwidth=\leftmarginii \advance\labelwidth-\labelsep
}{\end{enumerate}}

%% listings of short examples
%% the same as \enumerateA
\newenvironment{enumerateb}{}{}
\let\enumerateb\enumerateA
\let\endenumerateb\endenumerateA

%% listings of long examples
%% the same as \enumerateb but
%% add a little vertical space between the items
\newenvironment{enumerateB}{%
\begin{enumerateb}%
\addtolength{\itemsep}{\smallskipamount}%
}{\end{enumerateb}}

\newcommand{\itemJP}[1]{\relax\item #1.\enspace\ignorespaces}
\newcommand{\itemJPone}[1]{#1.\enspace\ignorespaces}

%% Exercises
%% This is like the xcb-environment of amsbook.cls
\newenvironment{Exercises}
{\bigbreak\specialsection*{Exercises}%
  \settowidth{\leftmargini}{00.\hskip\labelsep}%
  \settowidth{\leftmarginii}{(d.)\hskip\labelsep}%
  \enumerate
  \renewcommand{\labelenumi}{\theenumi.}
}{\endenumerate}

%% In chapter 10 we have only one poor Exercise
\newenvironment{Exercise}
{\bigbreak\specialsection*{Exercise}%
  \settowidth{\leftmargini}{00.\hskip\labelsep}%
  \settowidth{\leftmarginii}{(d.)\hskip\labelsep}%
  \enumerate
  \renewcommand{\labelenumi}{\theenumi.}
}{\endenumerate}

%% listings inside an exercise
\newenvironment{enumerateE}{}{}
\let\enumerateE\enumerate
\let\endenumerateE\endenumerate

\newcommand{\Hint}[1][Hint]{\emph{#1}: \ignorespaces}

%% In Notes \itemN has one  argument. It inserts \S "." and a sapce
%% \itemNN inserts \S\S
%% \itemNChapTen appears only in boi-10.tex
%%\newcommand{\beforeitemN}{\medbreak\noindent\indent}
\newcommand{\beforeitemN}{\vskip 0pt plus 1pt}
\newcommand{\afteritemN}{.\enspace\ignorespaces}
\newcommand{\itemN}[1]{\beforeitemN\S#1\afteritemN}
\newcommand{\itemNN}[1]{\beforeitemN\Sorig\S#1\afteritemN}
\newcommand{\itemNChapTen}[1]{%
  \beforeitemN#1\enspace\ignorespaces}
\newenvironment{Notes}{\bigbreak\specialsection*{Notes}%
\parskip=0pt plus 1pt\relax}{\par}

%% sublistings in Notes
%% the same as \enumerateT
\newenvironment{enumerateNn}{\listisep=0pt%
\begin{enumerateT}}{\end{enumerateT}}

\newenvironment{enumerateNnn}{
\renewcommand{\theenumii}{\roman{enumii}}
\begin{enumerate}}{\end{enumerate}}

%% This is appears only once in boi-8.tex.
\newcommand{\itemBb}[1][]{\par#1:\enspace\ignorespaces}
\newenvironment{enumerateBb}{}{\par}

%% Tits's resume in chap.9
\newenvironment{Tits}{\bigbreak\small\narrower}%
{\message{*** Look at the page break in Tits's resume ***^^J}%
  \bigbreak}

%%% Displays, diagrams, etc

%% no fullwidth in diplays (e.g., in standard \item-lists)
\def\fullwidthdisplay{}

%% centered cases edited from amstex.sty
\newenvironment{casesc}
{\left\{\def\arraystretch{1.2}\hskip-\arraycolsep \array{c@{\quad}l}}
  {\endarray\hskip-\arraycolsep\right.}

%% enumerate aligned equations:
%% see boi-8.tex for an example
\newcounter{eqalignnumcnt}
\newenvironment{eqalignnum}{\setcounter{eqalignnumcnt}0%
  \renewcommand{\theeqalignnumcnt}{\arabic{eqalignnumcnt}}%
  \renewcommand{\@currentlabel}{\theeqalignnumcnt}%
  \renewcommand{\intertext}[1]{\noalign{\vspace{1ex}%
      \advance\baselineskip-1ex\noindent##1}}%
  \par %
  \advance\baselineskip1ex
  \def\\{\cr}%
  \halign to\hsize \bgroup\addtocounter{eqalignnumcnt}1%
  \noindent\textup{(\theeqalignnumcnt)}##\tabskip=0ptplus1fil&\tabskip=0pt
  \hfill$##$&${}##$\hfill\tabskip=0ptplus1fil\cr}
{\crcr\egroup\vspace{1ex}\par\noindent\endtrivlist}

%% To give sometimes explicit non-bold eq-numbers
%% see boi-8.tex for usage
\newenvironment{equationleqno}[1][???]{%
  \renewcommand{\@currentlabel}{#1}
  \newcommand{\thist@g}{\textup{(\ignorespaces#1\unskip)}}$$}
{\leqno\thist@g$$\global\@ignoretrue}

%% commutative diagrams.
%% edited from amscd.sty, to avoid some messages
\atdef@>#1>#2>{\ampersand@
  \ifCD@ \global\bigaw@\minCDarrowwidth \else \global\bigaw@\minaw@ \fi
  \setboxz@h{$\m@th\scriptstyle\;{#1}\;\;$}%
  \ifdim\wdz@>\bigaw@\global\bigaw@\wdz@\fi
  \@ifnotempty{#2}{\setbox\@ne\hbox{$\m@th\scriptstyle\;{#2}\;\;$}%
    \ifdim\wd\@ne>\bigaw@\global\bigaw@\wd\@ne\fi}%
 \ifCD@\enskip\fi
%%   \mathrel{\mathop{\hbox to\bigaw@{\rightarrowfill@\displaystyle}}%
   \mathrel{\mathop{\hbox to\bigaw@{\hss\rightarrowfill@\displaystyle}}%
     \limits^{#1}\@ifnotempty{#2}{_{#2}}}%
 \ifCD@\enskip\fi \ampersand@}

%% cd-environment: shorter arrows for wide diagrams (in chap.7)
%% one optional argument: stretchfactor for longrightarrow
\newenvironment{cd}[1][1]{\setbox0\hbox{$\longrightarrow$}%
  \minCDarrowwidth #1\wd0 \begin{CD}}{\end{CD}}

%% tables of root systems in chap.6
\newcommand{\hcenter}[1]{{\leavevmode\setbox0\hbox{#1}\kern-.5\wd0\box0}}
\newenvironment{roottable}[2]{%
  \bigbreak{\bfseries #1. }#2
  \nopagebreak \medskip
  \par
  \noindent
  \mathsurround=0pt
  \setlength{\unitlength}{0.5ex}%
  \renewcommand{\arraystretch}{1.3}%
  \roottableaux}{}
\newenvironment{roottableEXC}[1]{%
  \message{*** Look at the page break in the table of rootsystems ***^^J}%
  \bigbreak{\bfseries #1. }
  \nopagebreak \medskip
  \par
  \noindent
  \mathsurround=0pt
  \setlength{\unitlength}{0.5ex}%
  \renewcommand{\arraystretch}{1.3}%
  }{}
\newcommand{\roottableaux}[8]{%
  \begin{tabular}{@{}l@{\quad}l@{\quad}l}
    Root system  &:& #1 %
    Root lattice &:& #2 %
    Weight lattice &:& #3 %
    Simple roots &:& #4 %
    Dynkin diagram &:& #5 %
    $\Aut\bigl(\Dyn(\Phi)\bigr)$ &:& #6 %
    Dominant weights &:& #7 %
    Minimal weights &:& #8 %
  \end{tabular}}

%% A very expensive macro for the iterated cases in chap.3, exerc.10
\newcommand{\casesspecial}[7]{\[
\def\arraystretch{1.2}
#1=
\left\{
\vphantom{
\array{l@{\quad}l@{\quad}l}
#2&\text{if}\smash[t]{\begin{cases}#3\\#4\end{cases}}\vadjust{\vspace{1ex}}\\
#5&\text{if}\smash[b]{\begin{cases}#6\\#7\end{cases}}\\
\endarray}
\right.
\hskip-\arraycolsep\array{l@{\quad}l@{\quad}l}
#2&\text{if}\begin{cases}#3\\#4\end{cases}\vadjust{\vspace{1ex}}\\
#5&\text{if}\begin{cases}#6\\#7\end{cases}\\
\endarray\hskip-\arraycolsep
\]}
%% Maybe this too artificial? Then change back:
%%\renewcommand{\casesspecial}[7]{
%%  \begin{alignat*}2
%%    #1&=#2&\quad&\text{if }\begin{cases}#3\\#4\end{cases}\\[1ex]
%%    #1&=#5&&\text{if }\begin{cases}#6\\#7\end{cases}
%%  \end{alignat*}}

%%  end of environ.sty

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "boi"
%%% End: 
